Benchmarking Quantum Surrogate Models on Scarce and Noisy Data

Surrogate models are ubiquitously used in industry and academia to efficiently approximate given black box functions. As state-of-the-art methods from classical machine learning frequently struggle to solve this problem accurately for the often scarce and noisy data sets in practical applications, investigating novel approaches is of great interest. Motivated by recent theoretical results indicating that quantum neural networks (QNNs) have the potential to outperform their classical analogs in the presence of scarce and noisy data, we benchmark their qualitative performance for this scenario empirically. Our contribution displays the first application-centered approach of using QNNs as surrogate models on higher dimensional, real world data. When compared to a classical artificial neural network with a similar number of parameters, our QNN demonstrates significantly better results for noisy and scarce data, and thus motivates future work to explore this potential quantum advantage in surrogate modelling. Finally, we demonstrate the performance of current NISQ hardware experimentally and estimate the gate fidelities necessary to replicate our simulation results.

==> txt/colorVersions.tex <==

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/heatmap_coldWarm.eps}
\caption{Delta\_R2 obtained by subtracting the CNN R2 score from the QNN R2 Score for different noise levels (x-axis) and sample sizes (y-axis).}
\label{fig_heatmap_coldwarm_CV}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/heatmap_blues.eps}
\caption{Delta\_R2 obtained by subtracting the CNN R2 score from the QNN R2 Score for different noise levels (x-axis) and sample sizes (y-axis).}
\label{fig_heatmap_blues}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/heatmap_greens.eps}
\caption{Delta\_R2 obtained by subtracting the CNN R2 score from the QNN R2 Score for different noise levels (x-axis) and sample sizes (y-axis).}
\label{fig_heatmap_greens}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/heatmap_YlGnBu.eps}
\caption{Delta\_R2 obtained by subtracting the CNN R2 score from the QNN R2 Score for different noise levels (x-axis) and sample sizes (y-axis).}
\label{fig_heatmap_YlGnBu}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/heatmap_bones.eps}
\caption{Delta\_R2 obtained by subtracting the CNN R2 score from the QNN R2 Score for different noise levels (x-axis) and sample sizes (y-axis).}
\label{fig_heatmap_bones}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/heatmap_reds.eps}
\caption{Delta\_R2 obtained by subtracting the CNN R2 score from the QNN R2 Score for different noise levels (x-axis) and sample sizes (y-axis).}
\label{fig_heatmap_reds}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/heatmap_viridis.eps}
\caption{Delta\_R2 obtained by subtracting the CNN R2 score from the QNN R2 Score for different noise levels (x-axis) and sample sizes (y-axis).}
\label{fig_heatmap_viridis}
\end{figure}



\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/R2_Diff_lines.eps}
\caption{Delta\_R2 obtained by subtracting the CNN R2 score from the QNN R2 Score for various sample sizes. The R2 Scores achieved by the QNN are higher than the R2 Scores achieved by the CNN for noise levels of 0.4 and higher. For sample sizes of 10 and 20 per dimension, the R2 Scores of the QNN are higher already at a noise level of 0.3.}
\label{fig_R2_Diff_lines_CV}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/R2_Diff_lines_colorblind.eps}
\caption{Delta\_R2 obtained by subtracting the CNN R2 score from the QNN R2 Score for various sample sizes. The R2 Scores achieved by the QNN are higher than the R2 Scores achieved by the CNN for noise levels of 0.4 and higher. For sample sizes of 10 and 20 per dimension, the R2 Scores of the QNN are higher already at a noise level of 0.3.}
\label{fig_R2_Diff_lines_colorblind}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/R2_Diff_lines_blues.eps}
\caption{Delta\_R2 obtained by subtracting the CNN R2 score from the QNN R2 Score for various sample sizes. The R2 Scores achieved by the QNN are higher than the R2 Scores achieved by the CNN for noise levels of 0.4 and higher. For sample sizes of 10 and 20 per dimension, the R2 Scores of the QNN are higher already at a noise level of 0.3.}
\label{fig_R2_Diff_lines_blues}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/R2_Diff_lines_greens.eps}
\caption{Delta\_R2 obtained by subtracting the CNN R2 score from the QNN R2 Score for various sample sizes. The R2 Scores achieved by the QNN are higher than the R2 Scores achieved by the CNN for noise levels of 0.4 and higher. For sample sizes of 10 and 20 per dimension, the R2 Scores of the QNN are higher already at a noise level of 0.3.}
\label{fig_R2_Diff_lines_greens}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/R2_Diff_lines_reds.eps}
\caption{Delta\_R2 obtained by subtracting the CNN R2 score from the QNN R2 Score for various sample sizes. The R2 Scores achieved by the QNN are higher than the R2 Scores achieved by the CNN for noise levels of 0.4 and higher. For sample sizes of 10 and 20 per dimension, the R2 Scores of the QNN are higher already at a noise level of 0.3.}
\label{fig_R2_Diff_lines_reds}
\end{figure}



\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/3d_surface_w_arrows.eps}
\caption{For individual datapoints of the Griewank function standardnormal noise multiplied by a factor of 0.5 is introduced. The top surface is generated by a CNN. The bottom surface is generated by a QNN. It becomes visible that the QNN can cope better with noise whereas the CNN shows overfitting tendencies.}
\label{fig_surfaces_CV}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/surface_blues.eps}
\caption{sample surface in different color scheme - to be inserted into plot with 3 surfaces once color scheme has been determined}
\label{fig_surface_blues}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/surface_bones.eps}
\caption{sample surface in different color scheme - to be inserted into plot with 3 surfaces once color scheme has been determined}
\label{fig_surface_bones}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/surface_coldWarm.eps}
\caption{sample surface in different color scheme - to be inserted into plot with 3 surfaces once color scheme has been determined}
\label{fig_surface_coldWarm}
\end{figure}


\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/surface_greens.eps}
\caption{sample surface in different color scheme - to be inserted into plot with 3 surfaces once color scheme has been determined}
\label{fig_surface_greens}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/surface_rainbow.eps}
\caption{sample surface in different color scheme - to be inserted into plot with 3 surfaces once color scheme has been determined}
\label{fig_surface_rainbow}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/surface_reds.eps}
\caption{sample surface in different color scheme - to be inserted into plot with 3 surfaces once color scheme has been determined}
\label{fig_surface_reds}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/surface_viridis.eps}
\caption{sample surface in different color scheme - to be inserted into plot with 3 surfaces once color scheme has been determined}
\label{fig_surface_viridis}
\end{figure}






\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/1dGriewank_belem.eps}
\caption{Original datapoints (sample size of 20) for a one-dimensional Griewank function and the surrogate function that has been obtained by running 100 iterations of 3 layers of our ansatz described in \ref{sec:concept} on ibmq\_belem.}
\label{fig_belem_CV}
\end{figure}


\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/1dGriewank_belem_darkblues.eps}
\caption{Original datapoints (sample size of 20) for a one-dimensional Griewank function and the surrogate function that has been obtained by running 100 iterations of 3 layers of our ansatz described in \ref{sec:concept} on ibmq\_belem.}
\label{fig_belem_darblues}
\end{figure}


\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/1dGriewank_belem_forestgreen.eps}
\caption{Original datapoints (sample size of 20) for a one-dimensional Griewank function and the surrogate function that has been obtained by running 100 iterations of 3 layers of our ansatz described in \ref{sec:concept} on ibmq\_belem.}
\label{fig_belem_forestgreen}
\end{figure}


\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/1dGriewank_belem_greys.eps}
\caption{Original datapoints (sample size of 20) for a one-dimensional Griewank function and the surrogate function that has been obtained by running 100 iterations of 3 layers of our ansatz described in \ref{sec:concept} on ibmq\_belem.}
\label{fig_belem_greys}
\end{figure}


\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/1dGriewank_belem_lightblues.eps}
\caption{Original datapoints (sample size of 20) for a one-dimensional Griewank function and the surrogate function that has been obtained by running 100 iterations of 3 layers of our ansatz described in \ref{sec:concept} on ibmq\_belem.}
\label{fig_belem_lightblues}
\end{figure}


\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/1dGriewank_belem_orangered.eps}
\caption{Original datapoints (sample size of 20) for a one-dimensional Griewank function and the surrogate function that has been obtained by running 100 iterations of 3 layers of our ansatz described in \ref{sec:concept} on ibmq\_belem.}
\label{fig_belem_orangered}
\end{figure}


\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/1dGriewank_belem_red.eps}
\caption{Original datapoints (sample size of 20) for a one-dimensional Griewank function and the surrogate function that has been obtained by running 100 iterations of 3 layers of our ansatz described in \ref{sec:concept} on ibmq\_belem.}
\label{fig_belem_red}
\end{figure}


\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{gfx/1dGriewank_belem_teal.eps}
\caption{Original datapoints (sample size of 20) for a one-dimensional Griewank function and the surrogate function that has been obtained by running 100 iterations of 3 layers of our ansatz described in \ref{sec:concept} on ibmq\_belem.}
\label{fig_belem_teal}
\end{figure}










